SPECTRE: Hybrid Ordinary-Parallel Speculative Serving for Resource-Efficient LLM Inference

LLM serving platforms are increasingly deployed as multi-model cloud systems, where user demand is often long-tailed: a few popular large models receive most requests, while many smaller tail models remain underutilized. We propose \textbf{SPECTRE} (Parallel \textbf{SPEC}ulative Decoding with a Multi-\textbf{T}enant \textbf{RE}mote Drafter), a serving framework that reuses underutilized tail-model services as remote drafters for heavily loaded large-model services through speculative decoding. SPECTRE enables draft generation and target-side verification to run in parallel, and makes such parallelism effective through three techniques: a hybrid ordinary-parallel speculative decoding strategy guided by a threshold derived from throughput analysis, speculative priority scheduling to preserve draft--target overlap under multi-tenant traffic, and draft-side prompt compression to reduce draft latency. We implement SPECTRE in \texttt{SGLang} and evaluate it across multiple draft--target model pairs, reasoning benchmarks, real-world long-context workloads, and a wide range of batch sizes. Results show that SPECTRE consistently improves large-model serving throughput while causing only minor interference to the native workloads of tail-model services. In large-model deployments, including Qwen3-235B-A22B with TP=8, SPECTRE achieves up to \textbf{2.28$\times$ speedup} over autoregressive decoding and up to an additional \textbf{66\% relative improvement} over the strongest speculative decoding baselines. Talk is cheap, we show you the code: https://github.com/sgl-project/sglang/pull/22272.

==> tex/03_analysis_old.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/pipeline3.pdf}
    \caption{
    Timeline comparison of ordinary speculative decoding, parallel speculative decoding, and SPECTRE. 
    Ordinary speculative decoding is fully serialized. 
    Parallel speculative decoding overlaps draft generation and target verification. 
    SPECTRE adaptively switches between parallel and ordinary coordination.
    }
    \label{fig:pipeline1}
\end{figure}

\section{Preliminary Throughput Analysis}
\label{sec:analysis}

In this section, we derive throughput models for ordinary and parallel speculative decoding, and identify the critical fallback ratio beyond which parallel speculative decoding becomes inferior. We then use this result to motivate the hybrid coordination strategy in \textbf{SPECTRE}.

\subsection{Setup}

We consider the decode stage of speculative decoding with batch size \(B\). Let \(T_D\) and \(T_T\) denote the latency of one draft-model forward pass and one target-model verification pass, respectively. We use \(L\) to denote the accepted length, and \(\gamma\) to denote the number of speculative tokens processed for one target-model verification request.
We assume
\begin{equation}
\gamma T_D < T_T.
\end{equation}
This assumption characterizes the condition under which speculative decoding admits the possibility of throughput gain: the draft model can prepare a speculative segment of length \(\gamma\) faster than the target model consumes it in one verification pass.

\subsection{Ordinary Speculative Decoding}

We first derive the throughput of ordinary speculative decoding (Fig.~\ref{fig:pipeline1} top case) as the reference for comparison with parallel speculative decoding. After initialization, each decoding round repeats the same pattern: the target model verifies a speculative segment of length \(\gamma\) and then produces one bonus token. Since that bonus token becomes the first token of the next speculative segment, the draft model only needs to generate \(\gamma-1\) new speculative tokens in each subsequent round.

Accordingly, each round incurs one target-model verification pass and \(\gamma-1\) draft-model token steps, yielding
\begin{equation}
T_{\mathrm{ord}} = T_T + (\gamma - 1)T_D,
\qquad
\mathrm{Thr}_{\mathrm{ord}}
=
\frac{B L}{T_{\mathrm{ord}}}
=
\frac{B L}{T_T + (\gamma-1)T_D}.
\label{eq:thr_ordinary}
\end{equation}

\subsection{Parallel Speculative Decoding}

We next derive the throughput of parallel speculative decoding (Fig.~\ref{fig:pipeline1} bottom case). After initialization, the draft model and the target model operate on different rounds concurrently: at round \(n\), the target model verifies the speculative segment prepared in round \(n-1\), while the draft model simultaneously prepares the speculative segment for round \(n+1\).

A key difference from ordinary speculative decoding is that the draft model must generate \(\gamma\) new speculative tokens in each round, rather than \(\gamma-1\). This is because the first token of the next speculative segment is generated before the target-side outcome of the current round becomes available, and therefore cannot be supplied in advance.

The throughput benefit of parallel speculative decoding comes from reusing the speculative segment prepared for the next round. Let \(r\) denote the fraction of requests whose prepared speculative segments become invalid due to verification mismatch. These requests cannot reuse the prepared continuation in the next round and therefore fall back to autoregressive decoding, contributing \(Br\) tokens per batch. The remaining fraction \(1-r\) can directly consume the prepared speculative segment and achieve an accepted length of \(L\), contributing \(B(1-r)L\) tokens per batch.

Therefore, the total number of output tokens per batch is
\begin{equation}
B\bigl[r + (1-r)L\bigr].
\end{equation}

Under the assumption \(\gamma T_D < T_T\), draft-side computation is fully overlapped by target-side verification, so the per-round latency is approximated by \(T_T\). The corresponding throughput is
\begin{equation}
T_{\mathrm{par}} \approx T_T,
\qquad
\mathrm{Thr}_{\mathrm{par}}
=
\frac{B\bigl[r + (1-r)L\bigr]}{T_{\mathrm{par}}}
\approx
\frac{B\bigl[r + (1-r)L\bigr]}{T_T}.
\label{eq:thr_parallel}
\end{equation}

\subsection{When Parallel Speculative Decoding Becomes Inferior}
\label{subsec: ordinary vs parallel}

We now compare Eq.~\eqref{eq:thr_ordinary} and Eq.~\eqref{eq:thr_parallel} to derive the condition under which parallel speculative decoding becomes inferior to ordinary speculative decoding. This occurs when
\begin{equation}
\mathrm{Thr}_{\mathrm{ord}} > \mathrm{Thr}_{\mathrm{par}}.
\end{equation}
Substituting the two throughput expressions gives
\begin{equation}
\frac{B L}{T_T + (\gamma-1)T_D}
>
\frac{B\bigl[r + (1-r)L\bigr]}{T_T}.
\end{equation}
Rearranging yields
\begin{equation}
r >
\frac{(\gamma-1)L T_D}
{\bigl(T_T + (\gamma-1)T_D\bigr)(L-1)}:= r^*.
\label{eq:r_threshold}
\end{equation}
Eq.~\eqref{eq:r_threshold} identifies the critical fallback ratio beyond which parallel speculative decoding becomes inferior. Once \(r\) exceeds this threshold, too many requests contribute only one auto-regressive token, and the throughput advantage of parallel speculative decoding is lost. 
This observation motivates SPECTRE to avoid committing to a single coordination mode and instead switch between parallel and ordinary execution according to the runtime fallback condition.

==> tex/A3_limitations.tex <==
\section{Limitations and Future Work}
\label{app:limitations}

SPECTRE benefits most when the draft and target models have strong token-level agreement. In our experiments, we therefore use small and large models from the same model family, which naturally provides compatible tokenization and similar next-token preferences. If the draft model comes from a very different family, the accepted length can decrease and reduce the realized speedup, although target-side verification still preserves the correctness of the final output. A natural direction for future work is to train or adapt a lightweight draft model through target-model distillation or agreement-aware fine-tuning, so that SPECTRE can support a broader range of draft--target pairs while retaining the same remote multi-tenant serving design.

